Logical Consistency and Greater Descriptive Power for Facial Hair Attribute Learning

Face attribute research has so far used only simple binary attributes for facial hair; e.g., beard / no beard. We have created a new, more descriptive facial hair annotation scheme and applied it to create a new facial hair attribute dataset, FH37K. Face attribute research also so far has not dealt with logical consistency and completeness. For example, in prior research, an image might be classified as both having no beard and also having a goatee (a type of beard). We show that the test accuracy of previous classification methods on facial hair attribute classification drops significantly if logical consistency of classifications is enforced. We propose a logically consistent prediction loss, LCPLoss, to aid learning of logical consistency across attributes, and also a label compensation training strategy to eliminate the problem of no positive prediction across a set of related attributes. Using an attribute classifier trained on FH37K, we investigate how facial hair affects face recognition accuracy, including variation across demographics. Results show that similarity and difference in facial hairstyle have important effects on the impostor and genuine score distributions in face recognition. The code is at https:// github.com/ HaiyuWu/ LogicalConsistency.

==> Algorithm/Training_algorithm.tex <==
\begin{listing}[h]
\centering
\begin{minted}{python}
for i in range(self.epoch):
    self.model.train()
    for j, (inputs, labels) in self.train_loader:
        inputs, labels = inputs.cuda(), labels.cuda()
        self.opt.zero_grad()
        output = self.model(inputs)
        binary_output = self.label_compensation(output)
        loss = (1 - self.config.lmbda) * self.bceloss(output, labels) + self.config.lmbda * self.lcploss(binary_output)
        loss.backward()
\end{minted}
\caption{Part of the training code for using the LCPLoss and label compensation strategy.}
\label{code:train}
\end{listing}


\begin{listing}[h]
\centering
\begin{minted}{python}
with torch.no_grad():
    for j, (inputs, labels) in self.test_loader:
        inputs, labels = inputs.cuda(), labels.cuda()
        self.opt.zero_grad()
        prediction = self.model(images)
        predicted = self.label_compensation(prediction)
\end{minted}
\caption{Part of the testing code for using the label compensation strategy.}
\label{code:test}
\end{listing}

==> Algorithm/logic_relationships.tex <==
\begin{algorithm}
    \caption{Failed prediction detection}
	\begin{algorithmic}
        \STATE \textbf{Attribute groups}
	    \STATE \ \ \ \ \ \textit{Beard areas}: Clean Shaven, Chin Area, Side to Side, Info not Vis
	    \STATE \ \ \ \ \ \textit{Beard lengths}: 5 O'clock Shadow, Median, Long, Info not Vis
	    \STATE \ \ \ \ \ \textit{Mustache}: None, Isolated, Connected-to-beard, Info not Vis
	    \STATE \ \ \ \ \ \textit{Sideburns}: None, Present, Connected-to-beard, Info not Vis
	    \STATE \ \ \ \ \ \textit{Bald}: False, Top only, Sides only, Top and Sides, Info not Vis
	    \STATE \textbf{Fail conditions}
	    \STATE \ \ \ \ \ \textit{Mutually exclusive}:
	    \STATE \ \ \ \ \ \ \ \ \ \ 1. More than one positive predictions in Beard areas (except Info not Vis), Beard lengths (except Info not Vis)
        \STATE \ \ \ \ \ \ \ \ \ \ Mustache, Sideburns, Bald group
        \STATE \ \ \ \ \ \ \ \ \ \ 2. Clean Shaven + any of the Beard lengths/Mustache Connected-to-beard/Sideburns Connected-to-beard
        \STATE \ \ \ \ \ \ \ \ \ \ 3. Chin area + Sideburns Connected-to-beard
        \STATE \ \ \ \ \ \ \ \ \ \ 4. Bald (Top and Sides or Sides only) + having sideburns (Sideburns Present, Sideburns Connected-to-beard)
        \STATE \ \ \ \ \ \textit{Dependency}:
        \STATE \ \ \ \ \ \ \ \ \ \ 1. Having beard (Chin Area, Side to Side) + one of the beard lengths must be true
        \STATE \ \ \ \ \ \ \ \ \ \ 2. Mustache is connected to beard + !(Chin Area, Side to Side)
        \STATE \ \ \ \ \ \ \ \ \ \ 3. Sideburns is connected to beard + !Side to Side
        \STATE \ \ \ \ \ \textit{Collectively exhaustive}
        \STATE \ \ \ \ \ \ \ \ \ \ No positive prediction in Beard area/Beard lengths/Mustache/Sideburns/Bald
        \STATE \textbf{Impossible:} prediction fits any of the conditions in \textit{Mutually exclusive} and \textit{Dependency}
        \STATE \textbf{Incomplete:} prediction fits any of the conditions in \textit{Collectively exhaustive}
	\end{algorithmic}
    \label{algo:fail_detection}
\end{algorithm}


==> Image_tex/arcface_BA-test.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/W/arcface/arcface_WM_clean_shaven.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/B/arcface/arcface_BM_clean_shaven.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/I/arcface/arcface_IM_clean_shaven.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/A/arcface/arcface_AM_clean_shaven.png}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/W/arcface/arcface_WM_chin_area.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/B/arcface/arcface_BM_chin_area.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/I/arcface/arcface_IM_chin_area.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/A/arcface/arcface_AM_chin_area.png}
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/W/arcface/arcface_WM_side2side.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/B/arcface/arcface_BM_side2side.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/I/arcface/arcface_IM_side2side.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/A/arcface/arcface_AM_side2side.png}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \begin{subfigure}[b]{0.49\linewidth}
                        \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/W/arcface/arcface_WM_double.png}
                    \end{subfigure}
                    \begin{subfigure}[b]{0.49\linewidth}
                        \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/B/arcface/arcface_BM_double.png}
                    \end{subfigure}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \begin{subfigure}[b]{0.49\linewidth}
                        \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/I/arcface/arcface_IM_double.png}
                    \end{subfigure}
                    \begin{subfigure}[b]{0.49\linewidth}
                        \includegraphics[width=\linewidth]{Images/Demographic_analysis/BA-test/A/arcface/arcface_AM_double.png}
                    \end{subfigure}
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
    \end{subfigure}
   \caption{Facial hair attribute based genuine and impostor distributions for WM, BM, IM, AM in BA-test dataset. First row is CS focused plots, second is CA focused plots,  third is S2S focused, and last row is same-beard-area focused plots. The feature extractor is ArcFace.}
\label{fig:facial_hair_demographic_analysis-arcface-BA-test}
\end{figure*}

==> Image_tex/arcface_BUPT-B.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/W/arcface/arcface_WM_clean_shaven.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/B/arcface/arcface_BM_clean_shaven.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/I/arcface/arcface_IM_clean_shaven.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/A/arcface/arcface_AM_clean_shaven.png}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/W/arcface/arcface_WM_chin_area.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/B/arcface/arcface_BM_chin_area.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/I/arcface/arcface_IM_chin_area.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/A/arcface/arcface_AM_chin_area.png}
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/W/arcface/arcface_WM_side2side.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/B/arcface/arcface_BM_side2side.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/I/arcface/arcface_IM_side2side.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/A/arcface/arcface_AM_side2side.png}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \begin{subfigure}[b]{0.49\linewidth}
                        \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/W/arcface/arcface_WM_double.png}
                    \end{subfigure}
                    \begin{subfigure}[b]{0.49\linewidth}
                        \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/B/arcface/arcface_BM_double.png}
                    \end{subfigure}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \begin{subfigure}[b]{0.49\linewidth}
                        \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/I/arcface/arcface_IM_double.png}
                    \end{subfigure}
                    \begin{subfigure}[b]{0.49\linewidth}
                        \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/A/arcface/arcface_AM_double.png}
                    \end{subfigure}
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
    \end{subfigure}
   \caption{Facial hair attribute based genuine and impostor distributions for WM, BM, IM, AM in BUPT-B dataset. First row is CS focused plots, second is CA focused plots,  third is S2S focused, and last row is same-beard-area focused plots. The feature extractor is ArcFace.}
\label{fig:facial_hair_demographic_analysis-arcface-BUPT-B}
\end{figure*}

==> Image_tex/magface_BUPT-B.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/W/magface/magface_WM_clean_shaven.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/B/magface/magface_BM_clean_shaven.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/I/magface/magface_IM_clean_shaven.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/A/magface/magface_AM_clean_shaven.png}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/W/magface/magface_WM_chin_area.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/B/magface/magface_BM_chin_area.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/I/magface/magface_IM_chin_area.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/A/magface/magface_AM_chin_area.png}
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/W/magface/magface_WM_side2side.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/B/magface/magface_BM_side2side.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/I/magface/magface_IM_side2side.png}
                \end{subfigure}
                \begin{subfigure}[b]{0.24\linewidth}
                    \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/A/magface/magface_AM_side2side.png}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \begin{subfigure}[b]{0.49\linewidth}
                        \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/W/magface/magface_WM_double.png}
                    \end{subfigure}
                    \begin{subfigure}[b]{0.49\linewidth}
                        \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/B/magface/magface_BM_double.png}
                    \end{subfigure}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \begin{subfigure}[b]{0.49\linewidth}
                        \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/I/magface/magface_IM_double.png}
                    \end{subfigure}
                    \begin{subfigure}[b]{0.49\linewidth}
                        \includegraphics[width=\linewidth]{Images/Demographic_analysis/BUPT-B/A/magface/magface_AM_double.png}
                    \end{subfigure}
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
    \end{subfigure}
   \caption{Facial hair attribute based genuine and impostor distributions for WM, BM, IM, AM in BUPT-B dataset. First row is CS focused plots, second is CA focused plots,  third is S2S focused, and last row is same-beard-area focused plots. The feature extractor is MagFace.}
\label{fig:facial_hair_demographic_analysis-magface-BUPT-B}
\end{figure*}

==> Image_tex/sup_mat/BA_VIS_INV.tex <==
\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/CS/0_136952.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/CS/0_185584.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/CS/0_188678.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/CS/034542.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/CS/050649.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/CS/079698.jpg}
                \end{subfigure}
            \caption{Samples of the Info partial visible - Clean Shaven + Beard Area Info Not Vis.}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/CA/0_30080.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/CA/0_30084.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/CA/188909.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/CA/149220.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/CA/174963.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/CA/181482.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Samples of the Info partial visible  - Chin Area + Beard Area Info Not Vis.}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/S2S/0_162226.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/S2S/0_162283.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/S2S/0_3367.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/S2S/018737.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/S2S/075397.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_VIS_INV/S2S/080398.jpg}
                \end{subfigure}
            \caption{Samples of the Info partial visible  - Side to Side + Beard Area Info Not Vis.}
            \end{subfigure}
        \end{subfigure}
                \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/5oS/0_182686.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/5oS/0_251088.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/5oS/0_6187.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/5oS/0_8672.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/5oS/165271.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/5oS/149220.jpg}
                \end{subfigure}
            \caption{Samples of the Info partial visible - 5 O'clock Shadow + Beard Length Info Not Vis.}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/Short/0_128630.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/Short/0_177272.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/Short/0_222779.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/Short/0_226849.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/Short/0_256538.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/Short/0_338647.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Samples of the Info partial visible - Short + Beard Length Info Not Vis.}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/Medium/0_150513.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/Medium/0_159180.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/Medium/0_162145.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/Medium/0_169659.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/Medium/0_203921.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_VIS_INV/Medium/0_91619.jpg}
                \end{subfigure}
            \caption{Samples of the Info partial visible - Medium + Beard Length Info Not Vis.}
            \end{subfigure}
        \end{subfigure}
    \end{subfigure}
   \caption{Examples of the Info partially visible.}
\label{fig:partial_info_not_visible}
\end{figure*}

==> Image_tex/sup_mat/Bald.tex <==
\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_False/0_39319.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_False/001550.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_False/014057.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_False/026448.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_False/044496.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_False/100693.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Bald-False.}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_T/0_85023.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_T/034543.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_T/060128.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_T/085812.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_T/120422.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_T/139968.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Samples of the attribute Bald Top Only.}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_TS/001684.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_TS/010186.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_TS/118615.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_TS/126511.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_TS/181397.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_TS/187652.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Bald Top and Sides.}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_S/0_13145.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_S/0_13149.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_S/0_245521.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_S/002862.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_S/003407.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_S/020308.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Bald Sides Only.}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_INV/0_2171.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_INV/0_45454.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_INV/017679.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_INV/156499.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_INV/157292.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/B_INV/189425.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Bald Info Not Vis.}
            \end{subfigure}
        \end{subfigure}
    \end{subfigure}
   \caption{Examples of the Bald attributes.}
\label{fig:bald}
\end{figure*}

==> Image_tex/sup_mat/Beard_Length.tex <==
\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/5oS/004485.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/5oS/010490.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/5oS/026214.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/5oS/032190.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/5oS/058914.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/5oS/096948.jpg}
                \end{subfigure}
            \caption{Samples of the attribute 5 O'clock Shadow.}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Short/013005.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Short/028610.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Short/076770.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Short/079203.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Short/081403.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Short/103015.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Samples of the attribute Short.}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Medium/0_118364.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Medium/119802.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Medium/122756.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Medium/126111.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Medium/126447.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Medium/141296.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Medium.}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Long/0_101559.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Long/0_4157.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Long/110774.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Long/148585.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Long/163749.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/Long/165667.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Long.}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_INV/0_10324.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_INV/0_34206.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_INV/0_27328.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_INV/0_40380.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_INV/0_48506.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BL_INV/0_6277.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Beard Length Info Not Vis.}
            \end{subfigure}
        \end{subfigure}
    \end{subfigure}
   \caption{Examples of the Beard Length attributes.}
\label{fig:beard_length}
\end{figure*}

==> Image_tex/sup_mat/Beard_area.tex <==
\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/CS/0_9900.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/CS/002726.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/CS/014114.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/CS/015507.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/CS/067790.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/CS/086371.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Clean Shaven.}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/CA/006849.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/CA/009878.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/CA/024480.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/CA/024606.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/CA/026314.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/CA/052299.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Samples of the attribute Chin Area.}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S2S/0_235718.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S2S/0_97676.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S2S/190514.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S2S/123500.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S2S/125647.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S2S/197733.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Side to Side.}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_INV/0_12807.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_INV/0_137379.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_INV/0_32452.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_INV/0_4696.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_INV/0_6771.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/BA_INV/094051.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Beard Area Info Not Vis.}
            \end{subfigure}
        \end{subfigure}
    \end{subfigure}
   \caption{Examples of the Beard Area attributes.}
\label{fig:beard_area}
\end{figure*}

==> Image_tex/sup_mat/Mustache.tex <==
\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_None/0_11908.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_None/0_81526.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_None/004994.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_None/075470.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_None/116989.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_None/138425.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Mustache-None.}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_Isolated/0_157594.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_Isolated/0_230677.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_Isolated/001354.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_Isolated/006922.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_Isolated/006980.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_Isolated/015980.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Samples of the attribute Mustache-Isolated.}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_C2B/065496.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_C2B/066876.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_C2B/068408.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_C2B/069877.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_C2B/071571.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_C2B/083467.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Mustache Connected to Beard.}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_INV/0_147207.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_INV/0_259109.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_INV/0_37903.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_INV/0_5552.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_INV/002148.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/M_INV/066321.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Mustache Info Not Vis.}
            \end{subfigure}
        \end{subfigure}
    \end{subfigure}
   \caption{Examples of the Mustache attributes.}
\label{fig:mustache}
\end{figure*}

==> Image_tex/sup_mat/Side2Side.tex <==
\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_None/001633.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_None/005916.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_None/022488.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_None/046432.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_None/059898.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_None/069283.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Sideburns-None.}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/SP/004440.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/SP/016908.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/SP/079385.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/SP/105589.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/SP/105589.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/SP/105885.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Samples of the attribute Sideburns-Present.}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_C2B/0_41047.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_C2B/0_59901.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_C2B/006043.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_C2B/031851.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_C2B/037352.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_C2B/135735.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Sideburns Connected to Beard.}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_INV/0_2067.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_INV/0_36037.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_INV/0_44545.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_INV/0_50236.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_INV/052723.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{Images/sup_mat_samples_for_attributes/S_INV/068582.jpg}
                \end{subfigure}
            \caption{Samples of the attribute Sideburns Info Not Vis.}
            \end{subfigure}
        \end{subfigure}
    \end{subfigure}
   \caption{Examples of the Sideburns attributes.}
\label{fig:sideburns}
\end{figure*}

==> Tables/sup_mat_BUPT-B.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
BUPT-B &
  N$_{pairs}$ &
  AM &
  N$_{pairs}$ &
  IM &
  N$_{pairs}$ &
  BM &
  N$_{pairs}$ &
  WM \\ \hline
\multirow{2}{*}{(CA,CA)} &
  \multirow{2}{*}{20,023,701} &
  0.3106 &
  \multirow{2}{*}{5,650,812} &
  0.1077 &
  \multirow{2}{*}{11,600,143} &
  0.0124 &
  \multirow{2}{*}{69,315,624} &
  0.0469 \\ \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
 &
   &
  0.344 &
   &
  0.1166 &
   &
  0.0112 &
   &
  0.0435 \\ \hline
\multirow{2}{*}{(CA,CS)} &
  \multirow{2}{*}{135,322,667} &
  0.1212 &
  \multirow{2}{*}{42,724,509} &
  0.0762 &
  \multirow{2}{*}{63,921,210} &
  0.0076 &
  \multirow{2}{*}{65,111,816} &
  0.0265 \\ \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
 &
   &
  0.1357 &
   &
  0.0749 &
   &
  0.0072 &
   &
  0.0264 \\ \hline
\multirow{2}{*}{(CA,S2S)} &
  \multirow{2}{*}{4,592,669} &
  0.1763 &
  \multirow{2}{*}{29,576,598} &
  0.0875 &
  \multirow{2}{*}{29,684,747} &
  0.0085 &
  \multirow{2}{*}{97,099,372} &
  0.0362 \\ \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
 &
   &
  0.201 &
   &
  0.096 &
   &
  0.0089 &
   &
  0.0341 \\ \hline
\multirow{2}{*}{(CS,CS)} &
  \multirow{2}{*}{228,110,497} &
  0.1129 &
  \multirow{2}{*}{80,428,098} &
  0.1781 &
  \multirow{2}{*}{87,789,833} &
  0.0111 &
  \multirow{2}{*}{15,234,314} &
  0.0465 \\ \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
 &
   &
  0.1137 &
   &
  0.159 &
   &
  0.0102 &
   &
  0.0429 \\ \hline
\multirow{2}{*}{(CS,S2S)} &
  \multirow{2}{*}{15,511,399} &
  0.0711 &
  \multirow{2}{*}{111,629,961} &
  0.0469 &
  \multirow{2}{*}{81,693,502} &
  0.0073 &
  \multirow{2}{*}{45,573,411} &
  0.0189 \\ \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
 &
   &
  0.0796 &
   &
  0.051 &
   &
  0.0075 &
   &
  0.0185 \\ \hline
\multirow{2}{*}{(S2S,S2S)} &
  \multirow{2}{*}{259,663} &
  0.2045 &
  \multirow{2}{*}{38,505,245} &
  0.1898 &
  \multirow{2}{*}{18,893,399} &
  0.0281 &
  \multirow{2}{*}{33,893,992} &
  0.0606 \\ \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
 &
   &
  0.2465 &
   &
  0.1809 &
   &
  0.0278 &
   &
  0.0536 \\ \hline
\end{tabular}
\caption{False match rate and corresponding fraction of each beard area comparison group. For the false match rate and fraction of each category, top number is ArcFace model, bottom is MagFace.
}
\label{table:fmr-bupt}
\end{table*}

==> Tables/sup_mat_accuracy.tex <==
\begin{table}[t]
\centering
\begin{tabular}{cccccc|c|c|c|c|c|c}
\hline
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\rotatebox{90}{Clean Shaven}} &
  \multicolumn{1}{c|}{\rotatebox{90}{Chin Area}} &
  \multicolumn{1}{c|}{\rotatebox{90}{Side to Side}} &
  \multicolumn{1}{c|}{\rotatebox{90}{Beard area Info Not Vis}} &
  \rotatebox{90}{5 O'clock Shadow} &
  \rotatebox{90}{Short} &
  \rotatebox{90}{Medium} &
  \rotatebox{90}{Long} &
  \rotatebox{90}{Bread length Info Not Vis} &
  \rotatebox{90}{Mustache-None} &
  \rotatebox{90}{Mustache-Isolated} \\ \hline
\multicolumn{1}{c|}{Overall acc} &
  \multicolumn{1}{c|}{86.86} &
  \multicolumn{1}{c|}{87.46} &
  \multicolumn{1}{c|}{88.05} &
  \multicolumn{1}{c|}{92.28} &
  80.62 &
  83.44 &
  92.40 &
  96.75 &
  91.34 &
  86.26 &
  85.74 \\
\multicolumn{1}{c|}{Negative acc} &
  \multicolumn{1}{c|}{93.88} &
  \multicolumn{1}{c|}{91.41} &
  \multicolumn{1}{c|}{88.34} &
  \multicolumn{1}{c|}{96.11} &
  80.62 &
  94.32 &
  98.04 &
  97.27 &
  94.36 &
  91.24 &
  90.27 \\
\multicolumn{1}{c|}{Positive acc} &
  \multicolumn{1}{c|}{70.21} &
  \multicolumn{1}{c|}{71.14} &
  \multicolumn{1}{c|}{87.59} &
  \multicolumn{1}{c|}{76.05} &
  80.61 &
  55.42 &
  23.60 &
  78.81 &
  78.18 &
  77.36 &
  66.42 \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \hline
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\rotatebox{90}{Mustache Connected to Beard}} &
  \multicolumn{1}{c|}{\rotatebox{90}{Mustache Info Not Vis}} &
  \multicolumn{1}{c|}{\rotatebox{90}{Sideburns-None}} &
  \multicolumn{1}{c|}{\rotatebox{90}{Sideburns-present}} &
  \rotatebox{90}{Sideburns Connected to Beard} &
  \rotatebox{90}{Sideburns Info Not Vis} &
  \rotatebox{90}{Bald False} &
  \rotatebox{90}{Bald Top Only} &
  \rotatebox{90}{Bald Top and Sides} &
  \rotatebox{90}{Bald Sides Only} &
  \rotatebox{90}{Bald Info Not Vis} \\ \hline
\multicolumn{1}{c|}{Overall acc} &
  \multicolumn{1}{c|}{89.11} &
  \multicolumn{1}{c|}{93.11} &
  \multicolumn{1}{c|}{80.33} &
  \multicolumn{1}{c|}{86.05} &
  89.86 &
  88.94 &
  92.80 &
  95.46 &
  97.37 &
  98.57 &
  95.79 \\
\multicolumn{1}{c|}{Negative acc} &
  \multicolumn{1}{c|}{91.15} &
  \multicolumn{1}{c|}{94.75} &
  \multicolumn{1}{c|}{87.17} &
  \multicolumn{1}{c|}{88.61} &
  93.25 &
  92.39 &
  84.00 &
  96.44 &
  98.58 &
  98.96 &
  97.25 \\
\multicolumn{1}{c|}{Positive acc} &
  \multicolumn{1}{c|}{85.64} &
  \multicolumn{1}{c|}{74.57} &
  \multicolumn{1}{c|}{70.97} &
  \multicolumn{1}{c|}{70.77} &
  78.46 &
  75.57 &
  95.10 &
  78.17 &
  66.25 &
  0 &
  84.21 \\ \hline
\end{tabular}
\caption{Performance of the BCELoss + LCPLoss + label compensation strategy on the logically inconsistent predictions counted case.}
\label{sup_table:performance}
\end{table}

==> Tables/sup_mat_consistency_rate.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
Attributes                    & Consistency rate
 & Attributes                      & Consistency rate
 \\ \hline
Clean Shaven                 & 0.99                  & Mustache Connected to Beard  & 0.83                 \\ \hline
Chin Area                    & 0.92                  & Mustache Info Not Vis        & 0.99                  \\ \hline
Side to Side                & 0.93                 & Sideburns-None                 & 0.90                 \\ \hline
Beard area Info Not Vis   & 0.98                  & Sideburns-Present              & 0.92                  \\ \hline
5 O'clock Shadow           & 0.91                 & Sideburns Connected to Beard & 0.90                  \\ \hline
Short                         & 0.83                 & Sideburns Info Not Vis       & 0.94                  \\ \hline
Medium                        & 0.89                  & Bald False                     & 0.99                 \\ \hline
Long                          & 1                    & Bald Top Only                       & 0.98                  \\ \hline
Beard length Info Not Vis & 0.98                  & Bald Top and Sides                 & 1                  \\ \hline
Mustache-None                & 0.98                 & Bald Sides Only                     & 1                    \\ \hline
Mustache-Isolated                      & 0.84                 & Bald Info Not Vis            & 0.99                  \\ \hline
\end{tabular}
\caption{The estimated consistency rate of each attribute in the FH37K dataset.}
\label{sup_table:consistency_rate}
\end{table*}


==> Tables/supplemental_material_number_of_samples.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
Attributes                    & \# of positive samples & Attributes                      & \# of positive samples \\ \hline
Clean Shaven                 & 9,562                  & Mustache Connected to Beard  & 15,887                 \\ \hline
Chin Area                    & 9,381                  & Mustache Info Not Vis        & 1,343                  \\ \hline
Side to Side                & 17,375                 & Sideburns-None                 & 14,004                 \\ \hline
Beard area Info Not Vis   & 3,001                  & Sideburns-Present              & 7,361                  \\ \hline
5 O'clock Shadow           & 11,759                 & Sideburns Connected to Beard & 9,809                  \\ \hline
Short                         & 11,693                 & Sideburns Info Not Vis       & 6,391                  \\ \hline
Medium                        & 2,475                  & Bald False                     & 31,085                 \\ \hline
Long                          & 747                    & Bald Top Only                       & 1,065                  \\ \hline
Beard length Info Not Vis & 2,757                  & Bald Top and Sides                 & 1,321                  \\ \hline
Mustache-None                & 10,228                 & Bald Sides Only                     & 161                    \\ \hline
Mustache-Isolated                      & 10,107                 & Bald Info Not Vis            & 3,933                  \\ \hline
\end{tabular}
\caption{Statistic information of the FH37K dataset.}
\label{sup_table:number_of_samples}
\end{table*}
